Make Your Training Flexible: Towards Deployment-Efficient Video Models

Popular video training methods mainly operate on a fixed number of tokens sampled from a predetermined spatiotemporal grid, resulting in sub-optimal accuracy-computation trade-offs due to inherent video redundancy. They also lack adaptability to varying computational budgets for downstream tasks, hindering applications of the most competitive model in real-world scenes. We thus propose a new test setting, Token Optimization, for maximized input information across budgets, which optimizes the size-limited set of input tokens through token selection from more suitably sampled videos. To this end, we propose a novel augmentation tool termed Flux. By making the sampling grid flexible and leveraging token selection, it is easily adopted in most popular video training frameworks, boosting model robustness with nearly no additional cost. We integrate Flux in large-scale video pre-training, and the resulting FluxViT establishes new state-of-the-art results across extensive tasks at standard costs. Notably, with 1/4 tokens only, it can still match the performance of previous state-of-the-art models with Token Optimization, yielding nearly 90\% savings. All models and data are available at https://github.com/OpenGVLab/FluxViT.

==> once4all_tables/iv2_s_k400.tex <==
\begin{table}[t]
    \centering
    % \setlength\tabcolsep{3.0pt}
    \setlength\tabcolsep{1.1pt}
    \resizebox{0.95\linewidth}{!}{
    \begin{tabular}{l|r|c|c|c|c|c}
    \Xhline{1.0pt}	
    \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Input Size}}&\multicolumn{4}{c|}{\textbf{Test Token Number}} & \multirow{2}{*}{\textbf{Avg}} \\ 
    ~ & ~ & 3072 & 2048 & 1024 & 512 & ~ \\
    \Xhline{0.8pt}
    ~ & 2$\times$224$^2$ & $\varnothing$ & $\varnothing$ & $\varnothing$ & 69.5 & 69.5\\
    ~ & 4$\times$224$^2$ & $\varnothing$ & $\varnothing$ & 80.5 & 73.6 & 77.1 \\
    ~ & \textbf{8$\times$224$^2$} & $\varnothing$ & 83.9 & 81.9 & 72.7 & 79.5 \\
    \multirow{-1}{*}{8$\times$224$^2$} & 12$\times$224$^2$ & 84.6 & 84.2 & 80.9 & 69.8 & 79.9 \\
    \multirow{1}{*}{Direct Tuned} & 16$\times$224$^2$ & 84.5 & 83.5 & 79.1 & 67.0 & 78.5 \\
    ~ & 20$\times$224$^2$ & 84.1 & 82.7 & 77.7 & 64.3 & 77.2 \\
    ~ & 24$\times$224$^2$ & 83.6 & 82.1 & 76.4 & 62.3 & 76.1 \\ \cline{2-7}
    ~ & \textbf{Avg} & 84.2 & 83.3 & 79.4 & 68.5 & - \\ \cline{3-7}
    ~ & \textbf{Max} & 84.6 & 84.3 & 81.9 & 73.6 & - \\ 
    \Xhline{0.8pt}	
    ~ & 2$\times$224$^2$ & $\varnothing$ & $\varnothing$ & $\varnothing$ & 68.1 & 68.1\\
    ~ & 4$\times$224$^2$ & $\varnothing$ & $\varnothing$ & 79.9 & 74.7 & 77.3 \\
    ~ & 8$\times$224$^2$ & $\varnothing$ & 84.3 & 82.7 & 76.7 & 81.2 \\
    ~ & 12$\times$224$^2$ & 85.1 & 85.1 & 82.8 & 75.8 & 82.2 \\
    2048 & 16$\times$224$^2$ & 85.4 & 85.2 & 82.6 & 75.3 & 82.1 \\
    Flux-Single Tuned & 20$\times$224$^2$ & 85.6 & 85.1 & 82.2 & 74.6 & 81.9 \\
    ~ & 24$\times$224$^2$ & 85.4 & 84.8 & 82.0 & 74.1 & 81.6 \\ \cline{2-7}
    ~ & \textbf{Avg} & 85.4 & 84.9 & 82.0 & 74.2 & - \\ \cline{3-7}
    ~ & \multirow{2}{*}{\textbf{Max}} & 85.6 & 85.2 & 82.8 & 76.7 & - \\ 
    ~ & ~ & \darkGreen{$\uparrow$\textbf{1.0}}  & \darkGreen{$\uparrow$\textbf{0.9}}  & \darkGreen{$\uparrow$\textbf{0.9}} & \darkGreen{$\uparrow$\textbf{3.1}} & - \\ 
    \Xhline{2pt}	
    ~ & 2$\times$224$^2$ & $\varnothing$  & $\varnothing$ & $\varnothing$ &  69.3 & 69.3 \\ 
    ~ & 4$\times$224$^2$ & $\varnothing$ & $\varnothing$ & 80.5 & 72.8 & 76.7 \\ 
    ~ & 8$\times$224$^2$ & $\varnothing$ & 83.9 & 81.9 & 72.7 & 79.5 \\ 
    \multirow{-1}{*}{12$\times$224$^2$} & \textbf{12$\times$224$^2$} & 84.9 & 84.3 & 80.9 & 67.8 & 79.4  \\ 
    \multirow{1}{*}{Direct Tuned} & 16$\times$224$^2$ & 84.8 & 83.9 & 78.9 & 65.2 & 78.2 \\
    ~ & 20$\times$224$^2$ & 84.6 & 83.4 & 77.6 & 62.4 & 77.0 \\
    ~ & 24$\times$224$^2$ & 84.3 & 82.6 & 76.4 & 60.4 & 75.9 \\\cline{2-7}
    ~ & \textbf{Avg} & 84.7 & 83.6 & 79.4 & 67.2 & - \\ \cline{3-7}
    ~ & \textbf{Max} & 84.9 & 84.3 & 81.9 & 72.8 & - \\ 
    \Xhline{0.8pt}	
    ~ & 2$\times$224$^2$ & $\varnothing$ & $\varnothing$ & $\varnothing$ & 72.2 & 72.2 \\
    ~ & 4$\times$224$^2$ & $\varnothing$ & $\varnothing$ & 81.0 & 79.3 & 80.2 \\
    ~ & 8$\times$224$^2$ & $\varnothing$ & 84.4 & 82.8 & 80.3 & 82.5 \\
    ~ & 12$\times$224$^2$ & 85.4 & 85.2 & 83.3 & 79.9 & 83.5 \\
    (3072, 2048, 1024) & 16$\times$224$^2$ & 85.7 & 85.1 & 83.5 & 79.2 & 83.4 \\
    Flux-Multi Tuned & 20$\times$224$^2$ & 85.7 & 85.3 & 83.0 & 78.9 & 83.2 \\
    ~ & 24$\times$224$^2$ & 85.6 & 85.0 & 82.7 & 78.2 & 82.9 \\ \cline{2-7}
    ~ & \textbf{Avg} & 85.6 & 85.0 & 82.7 & 78.3 & - \\ \cline{3-7}
    ~ & \multirow{2}{*}{\textbf{Max}} & 85.7 & 85.3 & 83.5 & 80.3 & - \\  
    ~ & ~ & \darkGreen{$\uparrow$\textbf{0.8}}  & \darkGreen{$\uparrow$\textbf{1.0}}  & \darkGreen{$\uparrow$\textbf{1.6}} & \darkGreen{$\uparrow$\textbf{7.5}} & - \\ 
    \Xhline{2pt}	
    \end{tabular}
    }
    % \vspace{-0.2cm}
    \vspace{-0.3cm}
    \caption{\textbf{Directly use Flux with InternVideo2-S on K400 Supervised Training.} Results are reported on K400 using 1clip$\times$1crop. All methods use K710 intermediate tuning.}
    \label{tab:ablations_multi_k400_iv2}
    \vspace{-0.2cm}
\end{table}

==> once4all_tables/once4all_mm_zs_action_recognition.tex <==
\begin{table}[tp]
    \centering
    \scriptsize
    \setlength{\tabcolsep}{0.5pt}
    \resizebox{\linewidth}{!}{
    \begin{tabu}{l|cc|cc|c|c}
        \Xhline{1pt}
        \multirow{2}*{\bf Model} & \multicolumn{2}{c|}{\textbf{K400}} & \multicolumn{2}{c|}{\textbf{K600}} & \multirow{2}*{\textbf{UCF101}} & \multirow{2}*{\textbf{MiTv1}} \\
        ~ & \scriptsize{Top-1} & \scriptsize{Top-5} & \scriptsize{Top-1} & \scriptsize{Top-5} & ~ & ~  \\
        \Xhline{0.8pt}
        Internvideo2-S~\cite{iv2} & 62.1 & 85.0 & 61.6 & 83.4 & 79.1 & 24.1 \\
        \hline
        EvaClip-B~\cite{eva_clip} & 57.4 & - & 57.0 & - & 68.6 & - \\
        Internvideo2-B~\cite{iv2} & 67.7 & 88.3 & 66.8 & 87.1 & 83.4 & 27.9 \\
        \Xhline{0.8pt}
        LanguageBind-L~\cite{zhu2023languagebind} & 64.0 & - & 61.9 & - & - & - \\
        EvaClip-L~\cite{eva_clip} & 65.0 & - & 64.9 & - & 76.8 & - \\
        Text4Vis-L~\cite{wu2023revisiting} & - & - & 68.9 & 90.3 & - & - \\
        Internvideo2-L~\cite{iv2} & 70.7 & 90.3 & 69.9 & 89.3 & 85.9 & 30.6 \\
        VideoCoCa-L~\cite{videococa} & 72.0 & 90.5 & 70.1 & 88.9 & 86.6 & - \\
        \Xhline{0.8pt}
        \textbf{FluxViT-S}$_{2048}$+  & \darkblue{67.0} & \darkblue{88.8} & \darkblue{65.5} & \darkblue{87.5} & \darkblue{87.5} & \darkblue{28.6} \\
        \textbf{FluxViT-S}$_{1024}$+  & \darkblue{65.6} & \darkblue{87.9} & \darkblue{64.3} & \darkblue{86.5} & \darkblue{87.2} & \darkblue{27.8} \\ 
        \textbf{FluxViT-S}$_{512}$+   & \darkblue{62.6} & \darkblue{85.5} & \darkblue{61.1} & \darkblue{84.2} & \darkblue{84.2} & \darkblue{26.5} \\ 
        \hline
        \textbf{FluxViT-B}$_{2048}$+  & \darkblue{70.7} & \darkblue{90.9} & \darkblue{69.3} & \darkblue{89.8} & \darkblue{89.1} & \darkblue{31.5} \\
        \textbf{FluxViT-B}$_{1024}$+  & \darkblue{69.6} & \darkblue{90.1} & \darkblue{68.3} & \darkblue{89.0} & \darkblue{89.1} & \darkblue{31.0} \\
        \textbf{FluxViT-B}$_{512}$+   & \darkblue{67.4} & \darkblue{87.4} & \darkblue{65.8} & \darkblue{87.7} & \darkblue{87.6} & \darkblue{29.8} \\
        \Xhline{1.0pt}
    \end{tabu}
    }
    \vspace{-0.2cm}
    \caption{\textbf{Zero-shot Action Recognition Results.} We only report the best results using flexible token sampling for our FluxViTs, as noted by ``FluxViT+'' in the table.
    }
    \label{tab:retrieval_zs_ar}
    % \vspace{-0.3cm}
\end{table}

==> once4all_tables/once4all_mm_zs_ar_full.tex <==
\begin{table}[tp]
    \centering
    \small
    \setlength{\tabcolsep}{3pt}
    \resizebox{\linewidth}{!}{
    \begin{tabu}{l|cc|cc|c|c}
        \toprule
        \multirow{2}*{\bf Method} & \multicolumn{2}{c|}{\textbf{K400}} & \multicolumn{2}{c|}{\textbf{K600}} & \multirow{2}*{\textbf{UCF101}} & \multirow{2}*{\textbf{MiTv1}} \\
        ~ & \textbf{Top1} & \textbf{Top5} & \textbf{Top1} & \textbf{Top5} & ~ & ~  \\
        \midrule
        \textbf{FluxViT}-S$_{2048}$+ & 67.0 & 88.8 & 65.5 & 87.5 & 87.5 & 28.6 \\ 
        \textbf{FluxViT}-S$_{2048}$+ & 67.0 & 88.8 & 65.5 & 87.5 & 87.5 & 28.6 \\ 
        \textbf{FluxViT}-S$_{1024}$+ & 65.6 & 87.9 & 64.3 & 86.5 & 87.2 & 27.8 \\ 
        \textbf{FluxViT}-S$_{1024}$+ & 65.6 & 87.9 & 64.3 & 86.5 & 87.2 & 27.8 \\ 
        \textbf{FluxViT}-S$_{512}$+  & 62.6 & 85.5 & 61.1 & 84.2 & 84.2 & 26.5 \\ 
        \textbf{FluxViT}-S$_{512}$+  & 62.6 & 85.5 & 61.1 & 84.2 & 84.2 & 26.5 \\ 
        \midrule
        \textbf{FluxViT}-B$_{2048}$+ & 70.7 & 90.9 & 69.3 & 89.8 & 89.1 & 31.5 \\
        \textbf{FluxViT}-B$_{2048}$+ & 70.7 & 90.9 & 69.3 & 89.8 & 89.1 & 31.5 \\
        \textbf{FluxViT}-B$_{1024}$+ & 69.6 & 90.1 & 68.3 & 89.0 & 89.1 & 31.0 \\
        \textbf{FluxViT}-B$_{1024}$+ & 69.6 & 90.1 & 68.3 & 89.0 & 89.1 & 31.0 \\
        \textbf{FluxViT}-B$_{512}$+  & 67.4 & 87.4 & 65.8 & 87.7 & 87.6 & 29.8 \\
        \textbf{FluxViT}-B$_{512}$+  & 67.4 & 87.4 & 65.8 & 87.7 & 87.6 & 29.8 \\
        \bottomrule
    \end{tabu}
    }
    \vspace{-0.3cm}
    \caption{\textbf{Zero-shot Action Recognition Results.} We only report the best results using flexible token sampling for our FluxViTs, as noted by `FluxViT+` in the table.
    }
    \label{tab:retrieval_zs_ar}
    \vspace{-0.3cm}
\end{table}
